The High-Quality Wide Multi-Channel Attack (HQ-WMCA) database

The High-Quality Wide Multi-Channel Attack database (HQ-WMCA) database extends the previous Wide Multi-Channel Attack database(WMCA), with more channels including color, depth, thermal, infrared (spectra), and short-wave infrared (spectra), and also a wide variety of attacks.

==> Makefile <==
# Created by Andre Anjos <andre.anjos@idiap.ch>
# Tue 18 Apr 2017 11:50:17 CEST

# Builds the LaTeX project as a PDF document

TEXFILE=main.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex $(@:%.pdf=%.tex);

all: $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.blg
	@rm -vf *.aux *.glo *.dvi *.ps main.pdf *.out *.brf $(PDFFILE)

